Xova: Baseline-Dependent Time and Channel Averaging for Radio Interferometry

Xova is a software package that implements baseline-dependent time and channel averaging on Measurement Set data. The uv-samples along a baseline track are aggregated into a bin until a specified decorrelation tolerance is exceeded. The degree of decorrelation in the bin correspondingly determines the amount of channel and timeslot averaging that is suitable for samples in the bin. This necessarily implies that the number of channels and timeslots varies per bin and the output data loses the rectilinear input shape of the input data.

==> Makefile <==
# Example makefile to help you compile your ADASS proceedings
# but you really should read the ManuscriptInstructions.pdf or
# at least the README file. For some smart cookies the Makefile
# could be sufficient too.
#
# Version 12-oct-2020   Peter Teuben
#
# See also:  http://www.adass.org/instructions/ADASS2020.tar
#            https://adass2020.es/static/proc/ADASS2020.tar
#
# P = paper_id    your proceedings paper ID code (the one with the dash, not dot)
# V = version     your version # (1,2,..) since you can only upload unique files
# A = 1stauthor   your last name, e.g. Teuben
# E = email       your contact email for submission issues
# FIGS = *eps     your EPS figures

                    # put your paper_id here (with dash, not dot), e.g. P10-2
                    # or find your template on http://www.astro.umd.edu/~teuben/adass/papers/
P = ADASS_template
                    # keep incrementing this after each upload of your $(P)
V = 1
                    # First author (for Papercheck.py)
A = Teuben
                    # contact person email
E = teuben@gmail.com
		    # your EPS figures (can be blank, and must be base-named with $(P)_*.eps
FIGS = example.eps

# override P,V,A,E,FIGS with a "makedefs" file, this is where authors should edit, not this Makefile
-include makedefs

#  variables for proceeding editors (don't modify, for export, not for authors)
YEAR   = 2020
ATDIR  = ADASS$(YEAR)_author_template
FILES  = AdassChecks.py AdassConfig.py AdassIndex.py ADASS_template.tex \
	 Aindex.py FixUnprintable.py \
	 copyrightform.pdf example.bib example.eps \
	 Index.py manual2010.pdf ManuscriptInstructions.pdf PaperCheck.py \
	 README subjectKeywords.txt TexScanner.py \
	 ascl.py asclKeywords.txt \
	 adass2020.bib Makefile makedefs \
	 $(FILESASP)

#  probably don't change these either (or notify the editors you have a special paper case)
TAR_FILE  = $(P)_v$(V).tar.gz
ZIP_FILE  = $(P)_v$(V).zip
FILESPDF  = $(P).pdf copyrightform_$(P)_$(A).pdf
FILESTEX  = $(P).tex $(P).bib $(FIGS) makedefs
FILESASP  = asp2014.bst asp2014.sty
FILES4AR  = $(FILESTEX) $(FILESPDF)

# ensure current directory is in the PATH
export PATH := .:$(PATH)

help:
	@echo AUTHOR targets:
	@echo ---------------
	@echo all:   pdf check tar
	@echo pdf:
	@echo check:
	@echo clean:
	@echo overleaf:
	@echo tar:
	@echo zip:
	@echo
	@echo EDITOR targets:
	@echo ---------------
	@echo fix:
	@echo inc:
	@echo spell:
	@echo aindex:
	@echo words:
	@echo asp1:
	@echo index:   needs TERMS=
	@echo ascl:
	@echo ascl1:
	@echo ascl2:   needs CODE=
	@echo pdf2:
	@echo rsync:


all:	pdf check tar


# not for authors, for creator of the ADASS instruction tar file
export:
	rm -rf $(ATDIR)
	mkdir  $(ATDIR)
	cp -a $(FILES) $(ATDIR)
	echo Created on `date` by `whoami`  > $(ATDIR)/VERSION
	-git remote -v                     >> $(ATDIR)/VERSION
	-git branch                        >> $(ATDIR)/VERSION
	tar cf ADASS$(YEAR).tar $(ATDIR)

# copyright is now part of the tar/zip file, checksum (sum) is 13785
copyrightform_$(P)_$(A).pdf: copyrightform.pdf
	cp copyrightform.pdf copyrightform_$(P)_$(A).pdf
	@echo Now go edit your copyrightform_$(P)_$(A).pdf form

# these targets are for most common unix systems, but YMMV. Modify if you need
# let the editors know you have a better way for the next ADASS team
# ASP prefers the latex;latex;dvipdfm route

DVIPDF = dvipdf

pdf:	$(P).pdf
	@echo xdg-open $(P).pdf

$(P).pdf:  $(P).dvi $(FIGS)
	$(DVIPDF) $(P)

$(P).bib:                                  # bootstrap if you don't have one
	touch $(P).bib

$(P).dvi:  $(P).tex $(P).bib
	latex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	latex $(P)
	latex $(P)

# an alternative method (ASP does not recommend it)
pdflatex:
	pdflatex $(P)
	if [ -s $(P).bib ]; then bibtex $(P); fi
	pdflatex $(P)
	pdflatex $(P)

clean:
	rm -f $(P).dvi $(P).bbl $(P).blg $(P).pdf $(P).aux $(P).log $(P).out $(P).toc $(P)_inc.tex

check:
	PaperCheck.py $(P) $(A)

ENCODING =
fix:
	FixUnprintable.py  $(P).tex $(ENCODING)

inc:
	tex2inc.py $(P).tex > $(P)_inc.tex
	@tail -1 $(P)_inc.tex
	@cat $(P).toc

spell:
	aspell --mode=tex check $(P).tex
	@echo Share your ~/.aspell.en.pws  ~/.aspell.en.prepl

aspell:
	(cd ../..; $(MAKE) aspell)

dvi:
	latex $(P)

aindex:
	Aindex.py $(P)

DETEX = detex
words:
	$(DETEX) $(P).tex | grep -o -E '\w+' | tr '[A-Z]' '[a-z]' | sort | uniq -c | sort -n

#  could add a checksum on personal copyrightform - if it's 13785,it's bad.
tar:    $(FILES4AR) _checksum
	tar zcf $(TAR_FILE) $(FILES4AR)
	@echo submit with e.g.
	@echo ncftpput www.adass2020.es  $(P) $(TAR_FILE)


overleaf:    $(FILESTEX)
	rm -f $(ZIP_FILE)
	zip $(ZIP_FILE) $(FILESTEX) $(FILESASP)
	@echo You can now upload $(ZIP_FILE) as a new project into overleaf
	@echo After import, git clone this here, and move all the git tree files here.
	@echo "The git clone command is under overleaf's Menu"


_checksum: copyrightform_$(P)_$(A).pdf
	@echo Checksum test
	@sum copyrightform_$(P)_$(A).pdf

# for editors
asp1:
	(cd ../..; $(MAKE) asp1 PID=$(P); grep box asp1.log)
	@echo xdg-open ../../authors/$(P).pdf

TERMS = foobar
index:
	@echo Using TERMS=$(TERMS)
	(cd ../Author_Template; Index.py $(TERMS))

ssindex:
	@echo Generating ssindex list
	(cd ../Author_Template; ./ssindex-org.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ssindex2:
	@echo Generating scored ssindex list
	(cd ../Author_Template; ./ssindex-scored.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

index2:
	(cd ../adass_subject_recommender ; detex ../$(P)/$(P).tex |  PYTHONPATH=`pwd` bin/find_subjects.py -m 10 -j)

ascl:
	(cd ../Author_Template; ./ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)
# 	(cd ../Author_Template; ./ascl-new.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex)

ascl1:
	(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).tex | grep ooindex | sort | uniq -c)
	-detex $(P).tex > $(P).txt
	-(cd ../Author_Template; ascl.py ../../ADASSProceedings2020/papers/$(P)/$(P).txt | grep ooindex | sort | uniq -c)
	-grep ooindex $(P).tex

CODE = foobar
.PHONY: ascl2
ascl2:
        xdg-open https://ascl.net/$(CODE)

pdf2:   pdf asp1
	xdg-open $(P).pdf
	xdg-open ../../authors/$(P).pdf

rsync: $(P).bib
	rsync -av $(P)_inc.tex $(P).bib $(FIGS) ../../authors
	rm -f ../../authors/$(P)_inc.{bbl,blg}

